Learning Shared RGB-D Fields: Unified Self-supervised Pre-training for Label-efficient LiDAR-Camera 3D Perception

Constructing large-scale labeled datasets for multi-modal perception model training in autonomous driving presents significant challenges. This has motivated the development of self-supervised pretraining strategies. However, existing pretraining methods mainly employ distinct approaches for each modality. In contrast, we focus on LiDAR-Camera 3D perception models and introduce a unified pretraining strategy, NeRF-Supervised Masked Auto Encoder (NS-MAE), which optimizes all modalities through a shared formulation. NS-MAE leverages NeRF's ability to encode both appearance and geometry, enabling efficient masked reconstruction of multi-modal data. Specifically, embeddings are extracted from corrupted LiDAR point clouds and images, conditioned on view directions and locations. Then, these embeddings are rendered into multi-modal feature maps from two crucial viewpoints for 3D driving perception: perspective and bird's-eye views. The original uncorrupted data serve as reconstruction targets for self-supervised learning. Extensive experiments demonstrate the superior transferability of NS-MAE across various 3D perception tasks under different fine-tuning settings. Notably, NS-MAE outperforms prior SOTA pre-training methods that employ separate strategies for each modality in BEV map segmentation under the label-efficient fine-tuning setting. Our code is publicly available at https://github.com/Xiaohao-Xu/Unified-Pretrain-AD/ .

==> figs/fig_teaser.tex <==



==> figs/overview.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{images/overview.pdf}
  \caption{Overview of the approach. The backbone to pre-train produces latent vectors for each input point. At pre-training time, the latent vector is fed into a volumetric occupancy head that classifies query points as full or empty. At semantic training or test time, the same latent vectors are fed into a semantic head, e.g., for semantic segmentation or object detection.}
  \label{fig:overview}
\end{figure*}

==> figs/perturbed_robustness.tex <==
\begin{figure}[t!]
	\centering
 \includegraphics[width=0.48\textwidth]{figures/perturbed_robustness.pdf} 
 \vspace{-3mm}	\caption{\textbf{Quantitative comparisons on depth reconstruction quality} (measured by absolute relative error) on KITTI~\cite{kitti} $val$ set with varied perturbed ratios of the input image during evaluation. Here, perturbation is implemented with random masking.}
	\label{fig:perturbed_exp}
  \vspace{-2mm}
\end{figure}


==> figs/render_fig_bev.tex <==
\begin{figure}[t]
	\centering
 \includegraphics[width=0.48\textwidth]{figures/qualitative_bev.pdf} 
\vspace{-2mm}
\caption{\textbf{Qualitative results of bird's-eye-view (BEV) depth}, \textbf{\textit{i.e.}, BEV occupancy}, rendered from a viewpoint that is orthogonal to the road plane, on \nus ~\cite{nuscenes} $val$. \textbf{Zoom in to view better.}}
       \vspace{-2mm}
	\label{fig:render_bev}
\end{figure}


==> figs/render_fig_pers.tex <==
\begin{figure*}[t!]
	\centering
 \includegraphics[width=\textwidth]{figures/qualitative_pers.pdf}
\vspace{-5mm}
	\caption{\textbf{Qualitative results of perspective-view image and depth} on KITTI~\cite{kitti} $val$ set. }
	\label{fig:render_pers}
 %\vspace{-5mm}
\end{figure*}




==> figs/rendering_analysis.tex <==
\begin{figure}[t]
	\centering
 \includegraphics[width=0.48\textwidth]{figures/rendering_analysis.pdf} 
 %\vspace{-5mm}
	\caption{\textbf{Qualitative visualizations of the radiance terms in rendering equations} (\textit{c.f.} Sec.~\ref{Sec: Radiance Field Rendering}), including volume density $\sigma(t)$, accumulated transmittance $T(t)$, and their product $T(t)\sigma(t)$, of sampled rendering rays on KITTI~\cite{kitti} $val$. Here, the rendering view direction is orthogonal to the perspective-view image plane. }
	\label{fig:render_equation}
%\vspace{-3mm}
\end{figure}


==> src/1-introduction.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=0.48\textwidth]{NS-MAE/figures/motivation.pdf} 
	\caption{\textbf{Motivation of our unified pre-training framework for transferable multi-modal perception representation learning}. }
	\label{fig:teaser}
\end{figure}


\section{{Introduction}}


\IEEEPARstart{T}owards robust autonomous driving, multi-modal perception~\cite{waymo,harley2023simple}, which aims to sense the surrounding scene by extracting and fusing representations from diverse modalities, is a crucial research direction. Meanwhile, with the booming development of modern network architectures~\cite{Vaswani2017AttentionIA}, great efforts on transferable representation learning have been witnessed to relieve the appetite for data~\cite{he2022masked}. However, \textbf{pre-training for multi-modal perception is in its infancy.}

We first {review the widely-adopted {multi-stage fully-supervised training} paradigm for current advanced multi-modal perception models}~\cite{liang2022bevfusion,liu2022bevfusion,yang2022deepinteraction}. In this paradigm, the networks of Lidar and camera branches are first pre-trained separately in a fully-supervised learning way, and then the whole architecture is jointly fine-tuned. However, such a  paradigm is not scalable due to the {{scarcity of labels for supervision}}. Specifically, annotating paired images and extremely sparse Lidar point clouds for 3D perception can be cumbersome~\cite{FLAVA}, thus high-quality 3D labels are scarce. To relieve this problem, some pre-training methods have been raised for single-modal perception models~\cite{10273603,li2022simipu,CMKD,voxel-mae-wacv,voxel-mae,boulch2023also,yang2023gd} with either camera-only or Lidar-only inputs to enable label-efficient transfer. However, their optimization formulations are not unified and there is no work to explore transferable representation learning for advanced multi-modal perception models, \textit{e.g.}, BEVFusion~\cite{liu2022bevfusion}, which achieves high performance on 3D perception tasks. 



To this end, we go on to think about {\textbf{what should the ideal multi-modal perception pre-training framework for transferable representation learning be like?}} Inspired by successful pre-training frameworks for vision~\cite{he2022masked} and language~\cite{devlin2018bert}, apart from the effectiveness to boost performance, we argue that the following features are crucial:
\begin{itemize}
    \item \textbf{Unified}:  it should be generic to various settings, \textit{e.g.}, input modalities, architectures, and downstreams.
    \item \textbf{Scalable}: it should embrace the huge unlabeled yet valuable multi-modal data and potentially huge models.
    \item \textbf{Neat}:  it should possess a simple formulation to be adapted to more diverse modalities for perception.
\end{itemize}

With these high-level goals in mind, we decouple the design of the pre-training framework for multi-modal perception into two sub-problems: (1) \textbf{learning} transferable multi-modal representation; (2) \textbf{unifying} the optimization formulation for multi-modal representation.



    
    On one hand, to learn multi-modal representation in a self-supervised way, we get inspiration from the great success of Masked AutoEncoder~\cite{he2022masked,yang2023masked,bachmann2022multimae} (MAE) paradigm. Specifically, MAE~\cite{he2022masked} follows a mask-then-reconstruct paradigm and shows inspiring transferability on various downstream tasks. To take a step forward, we would like to explore the possibility of adapting MAE to learn transferable multi-modal perception representation, thus empowering advanced multi-modal perception models~\cite{liu2022bevfusion,liang2022bevfusion}.
     %\item 
     
     On the other hand, to unify the multi-modal representation optimization, Neural Radiance Field (NeRF)~\cite{aliev2020neural} provides a neat form to encode diverse physical properties, \textit{e.g.}, color and geometry, of the scene via differential neural volume rendering procedure. We consider NeRF as a useful building block for multi-modal perception pre-training for two reasons. Firstly, the imaging process of optical systems for perception, \textit{e.g.}, Lidar and camera, can be approximately modeled with rendering in the radiance field. Secondly, neural rendering unifies the multi-modal reconstruction via a neat and explainable physics formula. Thus, we introduce the rendering process of NeRF to perception pre-training, enabling unified multi-modal representation optimization.






Inspired by the remarkable attainments achieved by MAE and NeRF, we make a synergy of them and propose a unified self-supervised multi-modal perception pre-training framework (\name), which learns transferable multi-modal representations in a conceptually-neat formulation. As is shown in Fig.~\ref{fig:teaser}, we assemble the plug-and-play pre-training components (\textcolor{black}{blue} parts of Fig.~\ref{fig:teaser}) to a typical embedding network of multi-modal perception models~\cite{liu2022bevfusion} (black parts of Fig.~\ref{fig:teaser}). During the pre-training, we first conduct modality-specific masking operations for multi-modal inputs, \textit{i.e.}, images and Lidar point clouds, separately. Then, we send the corrupted modalities to the multi-modal embedding network for embedding extraction. Specifically, we extract the embeddings that are generated and fused in two crucial coordination, \textit{i.e.}, the world and the camera coordination, for perception models~\cite{li2022bevformer,philion2020lift}. Afterward, according to specific view directions and spatial sampling locations, the embeddings are further rendered into diverse projected modality feature maps via differential volume rendering. Finally, the rendered feature maps are supervised by original images and point clouds via reconstruction-based self-supervised optimization.

At last, we evaluate the transferability of multi-modal representation learned via \name{} for diverse multi-modal and single-modal perception models. 

In summary, this work has the following contributions:
\begin{itemize}
    \item We propose {\textbf{a novel self-supervised pre-training framework for multi-modal perception representation learning}}, \textit{i.e.}, \name, which is generic to both multi-modal and single-modal perception models.
    \item We enable both the \textbf{self-supervised learning} and \textbf{optimization unification} of transferable multi-modal representation via plug-and-play designs in the spirit of multi-modal reconstruction in neural radiance field.
    \item We employ \name{} to various advanced single-modal and multi-modal perception models and \textbf{verify the transferability of multi-modal representation derived via \name{}} on diverse 3D perception tasks with diverse amounts of fine-tuning data.
\end{itemize}

    


==> tables/ablation_single_stage_ft.tex <==
\renewcommand{\arraystretch}{0.3}
\begin{table}[t]
%\small
\resizebox{0.48\textwidth}{!}
	{
        \setlength{\tabcolsep}{2pt}
	\centering
	\begin{tabular}{l|c|cc|cc}
          \toprule
        \multirow{6}{*}{Method}  & \multirow{2}{*}{Pre-training}  &\multicolumn{2}{c|}{{Image: $128\times352$}}  &\multicolumn{2}{c}{{Image: $256\times704$}}     \\
         & \multirow{2}{*}{Type} &\multicolumn{2}{c|}{{\#LiDAR Sweep: 1}}  &\multicolumn{2}{c}{{\#LiDAR Sweep: 9}}     \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6} 
      %   \midrule
         & & \quad mAP & NDS & \quad mAP & NDS  
         \\  \midrule
          BEVFusion& No   & \quad{50.5} &{53.3} &\quad {60.8} &{64.1}  \\ 
          + iNet  &Fully-supervised  &\quad{51.4} &{54.1}      &\quad{62.8} &{65.3}     
         \\  
        + \name  & Self-supervised  & \quad\textbf{{51.5}} &\textbf{54.7}      & \quad\textbf{{63.0}} &\textbf{65.5} 
         \\          

        \bottomrule
	\end{tabular}
       }
        %\vspace{1mm}
	\caption{\textbf{Comparison to supervised pre-training for Multi-modal Perception} model (BEVFusion~\cite{liu2022bevfusion}) on the 3D object detection task on \nus{} \cite{Caesar2020nuScenesAM} $val$. + iNet indicates that the camera encoder is pre-trained on ImageNet~\cite{deng2009imagenet} in a fully-supervised way. 
 	}
\vspace{-5mm}
	\label{tab:nuscene_det_sup_train}
\end{table}
\renewcommand{\arraystretch}{0.6}
